Compression of Uniformly Distributed Unit Quaternions

Unit quaternions are widely used in computer graphics making their efficient compression critical for reducing memory consumption and bandwidth requirements. In this paper, we present a novel method for encoding uniformly distributed unit quaternions. Our thorough analysis of several quaternion parameterizations compares their theoretical error properties, quantization behavior, computational cost, and memory efficiency and provides both an analytical and empirical characterization. We show that an infinity-norm parameterization with our optimized warp function consistently offers the smallest maximum error and the best storage efficiency, at a decompression cost equal to or lower than that of parameterization methods found in practice. We demonstrate the practical benefits of the proposed approach in several graphics applications, including tangent-space normal mapping, skeletal animation with blend weights, and Gaussian splatting.

==> common/arxiv.tex <==
% Overrides of egpubl.cls for the arXiv version (make arxiv); loaded from common/commands.tex
% only if \ArxivVersion is defined.
\makeatletter
% No conference header (EUROGRAPHICS, guest editors, volume, number) on the title page
% and no "submitted to EUROGRAPHICS" in the footers.
\copyrightTextTitPag{}
\copyrightTextRunPag{}
\def\ps@titlepage{\let\@mkboth\@gobbletwo
  \let\@oddhead\@empty\let\@evenhead\@empty
  \let\@oddfoot\@empty\let\@evenfoot\@empty}
\let\@oddfoot\@empty
\let\@evenfoot\@empty
% The class sets the PDF subject and keywords to the conference and the journal.
\hypersetup{pdfsubject={}, pdfkeywords={}}
% The class's \appendix numbers only sections; number subsections, too (e.g., B.2.3).
\g@addto@macro\appendix{\setcounter{secnumdepth}{3}}
\makeatother


==> lists/glossary.tex <==
\newglossaryentry{Glossar}
{
    name=Glossar,
    plural=Glossare,
    description={"selbstständig oder als Anhang eines bestimmten Textes erscheinendes Wörterverzeichnis"}
}

==> lists/symbols.tex <==
\nomenclature[0]{\textbf{Symbol}}{\textbf{Bedeutung}}
\nomenclature{$c$}{Lichtgeschwindigkeit}
\nomenclature{$h$}{Planksches Wirkungsquantum}


==> tabs/Measurements2D.tex <==
% Generated by Measurements2D -- run this program to regenerate. Edits here will be overwritten.
% 32 Bit Double Precision
\definecolor{mcc30}{rgb}{0.760,0.709,0.848}
\definecolor{mcc50}{rgb}{0.860,0.842,0.916}
\definecolor{mcc60}{rgb}{0.918,0.914,0.937}
\definecolor{mcc10}{rgb}{0.963,0.922,0.871}
\definecolor{mcc00}{rgb}{0.990,0.868,0.738}
\definecolor{mcc20}{rgb}{0.990,0.868,0.738}
\definecolor{mcc40}{rgb}{0.963,0.764,0.622}
\definecolor{mcc31}{rgb}{0.760,0.709,0.848}
\definecolor{mcc51}{rgb}{0.860,0.842,0.916}
\definecolor{mcc61}{rgb}{0.918,0.914,0.937}
\definecolor{mcc11}{rgb}{0.963,0.922,0.871}
\definecolor{mcc01}{rgb}{0.990,0.868,0.738}
\definecolor{mcc21}{rgb}{0.990,0.868,0.738}
\definecolor{mcc41}{rgb}{0.963,0.764,0.622}
\definecolor{mcc32}{rgb}{0.760,0.709,0.848}
\definecolor{mcc52}{rgb}{0.885,0.875,0.933}
\definecolor{mcc62}{rgb}{0.885,0.875,0.933}
\definecolor{mcc12}{rgb}{0.940,0.940,0.940}
\definecolor{mcc22}{rgb}{0.997,0.894,0.767}
\definecolor{mcc02}{rgb}{0.997,0.894,0.767}
\definecolor{mcc42}{rgb}{0.963,0.764,0.622}
\definecolor{mcc33}{rgb}{0.760,0.709,0.848}
\definecolor{mcc53}{rgb}{0.885,0.875,0.933}
\definecolor{mcc63}{rgb}{0.885,0.875,0.933}
\definecolor{mcc13}{rgb}{0.940,0.940,0.940}
\definecolor{mcc23}{rgb}{0.997,0.894,0.767}
\definecolor{mcc03}{rgb}{0.997,0.894,0.767}
\definecolor{mcc43}{rgb}{0.963,0.764,0.622}
\definecolor{mcc04}{rgb}{0.760,0.709,0.848}
\definecolor{mcc24}{rgb}{0.843,0.820,0.905}
\definecolor{mcc14}{rgb}{0.903,0.897,0.935}
\definecolor{mcc34}{rgb}{0.940,0.940,0.940}
\definecolor{mcc64}{rgb}{0.978,0.909,0.825}
\definecolor{mcc44}{rgb}{0.986,0.851,0.719}
\definecolor{mcc54}{rgb}{0.963,0.764,0.622}
\definecolor{mcc25}{rgb}{0.760,0.709,0.848}
\definecolor{mcc05}{rgb}{0.843,0.820,0.905}
\definecolor{mcc15}{rgb}{0.903,0.897,0.935}
\definecolor{mcc65}{rgb}{0.940,0.940,0.940}
\definecolor{mcc35}{rgb}{0.978,0.909,0.825}
\definecolor{mcc45}{rgb}{0.986,0.851,0.719}
\definecolor{mcc55}{rgb}{0.963,0.764,0.622}
\definecolor{mcc26}{rgb}{0.760,0.709,0.848}
\definecolor{mcc66}{rgb}{0.843,0.820,0.905}
\definecolor{mcc46}{rgb}{0.903,0.897,0.935}
\definecolor{mcc56}{rgb}{0.940,0.940,0.940}
\definecolor{mcc06}{rgb}{0.978,0.909,0.825}
\definecolor{mcc16}{rgb}{0.986,0.851,0.719}
\definecolor{mcc36}{rgb}{0.963,0.764,0.622}
\definecolor{mcc17}{rgb}{0.760,0.709,0.848}
\definecolor{mcc27}{rgb}{0.843,0.820,0.905}
\definecolor{mcc67}{rgb}{0.903,0.897,0.935}
\definecolor{mcc47}{rgb}{0.940,0.940,0.940}
\definecolor{mcc57}{rgb}{0.978,0.909,0.825}
\definecolor{mcc07}{rgb}{0.986,0.851,0.719}
\definecolor{mcc37}{rgb}{0.963,0.764,0.622}

\footnotesize
\begin{tblr}{l cccc cc cc}
    \toprule
                         & \SetCell[c=4]{c}{Error $\downarrow$} &   &   &   & \SetCell[c=2]{c}{Compression $\downarrow$} &   & \SetCell[c=2]{c}{Decompression $\downarrow$} &   \\
                           \cmidrule[lr]{2-5}                                   \cmidrule[lr]{6-7}                                    \cmidrule[lr]{8-9}
                         & \SetCell[c=2]{c}{Maximum} &   & \SetCell[c=2]{c}{Average} &   &        &       &        &                    \\
                           \cmidrule[lr]{2-3}                     \cmidrule[lr]{4-5}
    Method               & Domain & Range & Domain & Range & Domain & Range & Unpack & $\mathrm{norm}_2$ \\
    \midrule
    $\lOne$ & \SetCell{bg=mcc00} $5.34\times10^{-8}$ \cmark & \SetCell{bg=mcc01} $5.34\times10^{-8}$ \cmark & \SetCell{bg=mcc02} $2.18\times10^{-8}$ & \SetCell{bg=mcc03} $2.18\times10^{-8}$ & \SetCell{bg=mcc04} $2.04$ & \SetCell{bg=mcc05} $16.5$ & \SetCell{bg=mcc06} $2.41$ & \SetCell{bg=mcc07} $4.53$ \\
    $\lTwoI$ & \SetCell{bg=mcc10} $5.33\times10^{-8}$ \cmark & \SetCell{bg=mcc11} $5.33\times10^{-8}$ \cmark & \SetCell{bg=mcc12} $2.12\times10^{-8}$ & \SetCell{bg=mcc13} $2.12\times10^{-8}$ & \SetCell{bg=mcc14} $5.54$ & \SetCell{bg=mcc15} $17.8$ & \SetCell{bg=mcc16} $2.57$ & \SetCell{bg=mcc17} $2.57$ \\
    $\lInf$ & \SetCell{bg=mcc20} $5.34\times10^{-8}$ \cmark & \SetCell{bg=mcc21} $5.34\times10^{-8}$ \cmark & \SetCell{bg=mcc22} $2.18\times10^{-8}$ & \SetCell{bg=mcc23} $2.18\times10^{-8}$ & \SetCell{bg=mcc24} $2.27$ & \SetCell{bg=mcc25} $14.9$ & \SetCell{bg=mcc26} $1.71$ & \SetCell{bg=mcc27} $3.76$ \\
    $\lInfT$ ($\tan$) & \SetCell{bg=mcc30} $4.19\times10^{-8}$ \cmark & \SetCell{bg=mcc31} $4.19\times10^{-8}$ \cmark & \SetCell{bg=mcc32} $2.09\times10^{-8}$ & \SetCell{bg=mcc33} $2.09\times10^{-8}$ & \SetCell{bg=mcc34} $6.77$ & \SetCell{bg=mcc35} $33.0$ & \SetCell{bg=mcc36} $4.64$ & \SetCell{bg=mcc37} $7.33$ \\
    $\lInfT$ (Remez3) & \SetCell{bg=mcc40} $1.16\times10^{-7}$ \xmark & \SetCell{bg=mcc41} $7.38\times10^{-8}$ \xmark & \SetCell{bg=mcc42} $3.31\times10^{-8}$ & \SetCell{bg=mcc43} $2.25\times10^{-8}$ & \SetCell{bg=mcc44} $10.5$ & \SetCell{bg=mcc45} $33.3$ & \SetCell{bg=mcc46} $1.84$ & \SetCell{bg=mcc47} $3.88$ \\
    $\lInfT$ (Remez5) & \SetCell{bg=mcc50} $4.21\times10^{-8}$ \cmark & \SetCell{bg=mcc51} $4.20\times10^{-8}$ \cmark & \SetCell{bg=mcc52} $2.10\times10^{-8}$ & \SetCell{bg=mcc53} $2.10\times10^{-8}$ & \SetCell{bg=mcc54} $16.6$ & \SetCell{bg=mcc55} $42.1$ & \SetCell{bg=mcc56} $2.01$ & \SetCell{bg=mcc57} $4.07$ \\
    $\lInfT$ (Remez3-Opt) & \SetCell{bg=mcc60} $4.29\times10^{-8}$ \xmark & \SetCell{bg=mcc61} $4.29\times10^{-8}$ \xmark & \SetCell{bg=mcc62} $2.10\times10^{-8}$ & \SetCell{bg=mcc63} $2.10\times10^{-8}$ & \SetCell{bg=mcc64} $10.4$ & \SetCell{bg=mcc65} $31.3$ & \SetCell{bg=mcc66} $1.75$ & \SetCell{bg=mcc67} $3.87$ \\
    \bottomrule
\end{tblr}


==> tabs/Measurements3D.tex <==
% Generated by Measurements3D -- run this program to regenerate. Edits here will be overwritten.
% 32 Bit Single Precision
\definecolor{mcc50}{rgb}{0.760,0.709,0.848}
\definecolor{mcc30}{rgb}{0.831,0.804,0.897}
\definecolor{mcc40}{rgb}{0.893,0.884,0.934}
\definecolor{mcc20}{rgb}{0.924,0.921,0.938}
\definecolor{mcc60}{rgb}{0.956,0.927,0.891}
\definecolor{mcc10}{rgb}{0.989,0.901,0.792}
\definecolor{mcc00}{rgb}{0.982,0.838,0.705}
\definecolor{mcc70}{rgb}{0.963,0.764,0.622}
\definecolor{mcc61}{rgb}{0.760,0.709,0.848}
\definecolor{mcc31}{rgb}{0.823,0.792,0.891}
\definecolor{mcc21}{rgb}{0.885,0.875,0.933}
\definecolor{mcc41}{rgb}{0.912,0.907,0.936}
\definecolor{mcc51}{rgb}{0.940,0.940,0.940}
\definecolor{mcc71}{rgb}{0.968,0.917,0.853}
\definecolor{mcc01}{rgb}{0.997,0.894,0.767}
\definecolor{mcc11}{rgb}{0.980,0.829,0.695}
\definecolor{mcc81}{rgb}{0.963,0.764,0.622}
\definecolor{mcc22}{rgb}{0.760,0.709,0.848}
\definecolor{mcc42}{rgb}{0.760,0.709,0.848}
\definecolor{mcc32}{rgb}{0.760,0.709,0.848}
\definecolor{mcc52}{rgb}{0.760,0.709,0.848}
\definecolor{mcc62}{rgb}{0.885,0.875,0.933}
\definecolor{mcc12}{rgb}{0.940,0.940,0.940}
\definecolor{mcc02}{rgb}{0.997,0.894,0.767}
\definecolor{mcc72}{rgb}{0.963,0.764,0.622}
\definecolor{mcc83}{rgb}{0.760,0.709,0.848}
\definecolor{mcc23}{rgb}{0.860,0.842,0.916}
\definecolor{mcc43}{rgb}{0.860,0.842,0.916}
\definecolor{mcc33}{rgb}{0.860,0.842,0.916}
\definecolor{mcc53}{rgb}{0.860,0.842,0.916}
\definecolor{mcc63}{rgb}{0.918,0.914,0.937}
\definecolor{mcc73}{rgb}{0.963,0.922,0.871}
\definecolor{mcc13}{rgb}{0.990,0.868,0.738}
\definecolor{mcc03}{rgb}{0.963,0.764,0.622}
\definecolor{mcc14}{rgb}{0.760,0.709,0.848}
\definecolor{mcc74}{rgb}{0.831,0.804,0.897}
\definecolor{mcc04}{rgb}{0.893,0.884,0.934}
\definecolor{mcc24}{rgb}{0.924,0.921,0.938}
\definecolor{mcc34}{rgb}{0.956,0.927,0.891}
\definecolor{mcc54}{rgb}{0.989,0.901,0.792}
\definecolor{mcc64}{rgb}{0.982,0.838,0.705}
\definecolor{mcc44}{rgb}{0.963,0.764,0.622}
\definecolor{mcc05}{rgb}{0.760,0.709,0.848}
\definecolor{mcc15}{rgb}{0.823,0.792,0.891}
\definecolor{mcc75}{rgb}{0.885,0.875,0.933}
\definecolor{mcc35}{rgb}{0.912,0.907,0.936}
\definecolor{mcc65}{rgb}{0.940,0.940,0.940}
\definecolor{mcc55}{rgb}{0.968,0.917,0.853}
\definecolor{mcc25}{rgb}{0.997,0.894,0.767}
\definecolor{mcc45}{rgb}{0.980,0.829,0.695}
\definecolor{mcc85}{rgb}{0.963,0.764,0.622}
\definecolor{mcc76}{rgb}{0.760,0.709,0.848}
\definecolor{mcc16}{rgb}{0.831,0.804,0.897}
\definecolor{mcc56}{rgb}{0.893,0.884,0.934}
\definecolor{mcc36}{rgb}{0.924,0.921,0.938}
\definecolor{mcc06}{rgb}{0.956,0.927,0.891}
\definecolor{mcc66}{rgb}{0.956,0.927,0.891}
\definecolor{mcc46}{rgb}{0.989,0.901,0.792}
\definecolor{mcc26}{rgb}{0.982,0.838,0.705}
\definecolor{mcc86}{rgb}{0.963,0.764,0.622}
\definecolor{mcc07}{rgb}{0.760,0.709,0.848}
\definecolor{mcc77}{rgb}{0.823,0.792,0.891}
\definecolor{mcc17}{rgb}{0.885,0.875,0.933}
\definecolor{mcc37}{rgb}{0.912,0.907,0.936}
\definecolor{mcc67}{rgb}{0.940,0.940,0.940}
\definecolor{mcc57}{rgb}{0.968,0.917,0.853}
\definecolor{mcc47}{rgb}{0.997,0.894,0.767}
\definecolor{mcc27}{rgb}{0.980,0.829,0.695}
\definecolor{mcc87}{rgb}{0.963,0.764,0.622}

\footnotesize
\begin{tblr}{l cccc cc cc}
    \toprule
                         & \SetCell[c=4]{c}{Error $\downarrow$} &   &   &   & \SetCell[c=2]{c}{Compression $\downarrow$} &   & \SetCell[c=2]{c}{Decompression $\downarrow$} &   \\
                           \cmidrule[lr]{2-5}                                   \cmidrule[lr]{6-7}                                    \cmidrule[lr]{8-9}
                         & \SetCell[c=2]{c}{Maximum} &   & \SetCell[c=2]{c}{Average} &   &        &       &        &                    \\
                           \cmidrule[lr]{2-3}                     \cmidrule[lr]{4-5}
    Method               & Domain & Range & Domain & Range & Domain & Range & Unpack & $\mathrm{norm}_2$ \\
    \midrule
    $\lTwoI$ & \SetCell{bg=mcc00} $0.00363$ \cmark & \SetCell{bg=mcc01} $0.00258$ \cmark & \SetCell{bg=mcc02} $0.00129$ & \SetCell{bg=mcc03} $0.00128$ & \SetCell{bg=mcc04} $4.83$ & \SetCell{bg=mcc05} $26.3$ & \SetCell{bg=mcc06} $3.96$ & \SetCell{bg=mcc07} $3.96$ \\
    $\lInf$ & \SetCell{bg=mcc10} $0.00301$ \cmark & \SetCell{bg=mcc11} $0.00301$ \cmark & \SetCell{bg=mcc12} $0.00126$ & \SetCell{bg=mcc13} $0.00125$ & \SetCell{bg=mcc14} $3.48$ & \SetCell{bg=mcc15} $29.5$ & \SetCell{bg=mcc16} $3.49$ & \SetCell{bg=mcc17} $4.75$ \\
    $\lInfT$ ($\tan$) & \SetCell{bg=mcc20} $0.00270$ \cmark & \SetCell{bg=mcc21} $0.00237$ \cmark & \SetCell{bg=mcc22} $0.00120$ & \SetCell{bg=mcc23} $0.00119$ & \SetCell{bg=mcc24} $11.9$ & \SetCell{bg=mcc25} $64.4$ & \SetCell{bg=mcc26} $7.74$ & \SetCell{bg=mcc27} $10.9$ \\
    $\lInfT$ (Remez3) & \SetCell{bg=mcc30} $0.00255$ \cmark & \SetCell{bg=mcc31} $0.00232$ \cmark & \SetCell{bg=mcc32} $0.00120$ & \SetCell{bg=mcc33} $0.00119$ & \SetCell{bg=mcc34} $16.7$ & \SetCell{bg=mcc35} $56.9$ & \SetCell{bg=mcc36} $3.76$ & \SetCell{bg=mcc37} $5.93$ \\
    $\lInfT$ (Remez5) & \SetCell{bg=mcc40} $0.00267$ \cmark & \SetCell{bg=mcc41} $0.00238$ \cmark & \SetCell{bg=mcc42} $0.00120$ & \SetCell{bg=mcc43} $0.00119$ & \SetCell{bg=mcc44} $31.3$ & \SetCell{bg=mcc45} $71.0$ & \SetCell{bg=mcc46} $4.07$ & \SetCell{bg=mcc47} $6.82$ \\
    $\lInfT$ (Remez3-Opt-Domain) & \SetCell{bg=mcc50} $0.00246$ \cmark & \SetCell{bg=mcc51} $0.00244$ \xmark & \SetCell{bg=mcc52} $0.00120$ & \SetCell{bg=mcc53} $0.00119$ & \SetCell{bg=mcc54} $17.0$ & \SetCell{bg=mcc55} $58.3$ & \SetCell{bg=mcc56} $3.74$ & \SetCell{bg=mcc57} $6.26$ \\
    $\lInfT$ (Remez3-Opt-Range) & \SetCell{bg=mcc60} $0.00287$ \xmark & \SetCell{bg=mcc61} $0.00221$ \cmark & \SetCell{bg=mcc62} $0.00121$ & \SetCell{bg=mcc63} $0.00120$ & \SetCell{bg=mcc64} $17.1$ & \SetCell{bg=mcc65} $58.2$ & \SetCell{bg=mcc66} $3.96$ & \SetCell{bg=mcc67} $6.22$ \\
    $\lOne^\star$ (ONV) & \SetCell{bg=mcc70} $0.00369$ \cmark & \SetCell{bg=mcc71} $0.00246$ \cmark & \SetCell{bg=mcc72} $0.00131$ & \SetCell{bg=mcc73} $0.00122$ & \SetCell{bg=mcc74} $3.92$ & \SetCell{bg=mcc75} $36.0$ & \SetCell{bg=mcc76} $2.36$ & \SetCell{bg=mcc77} $4.19$ \\
    SF &  & \SetCell{bg=mcc81} $0.0162$ \xmark &  & \SetCell{bg=mcc83} $0.00118$ &  & \SetCell{bg=mcc85} $202$ & \SetCell{bg=mcc86} $18.7$ & \SetCell{bg=mcc87} $18.7$ \\
    \bottomrule
\end{tblr}


==> tabs/Measurements4D.tex <==
% Generated by Measurements4D -- run this program to regenerate. Edits here will be overwritten.
\definecolor{mcc50}{rgb}{0.760,0.709,0.848}
\definecolor{mcc30}{rgb}{0.843,0.820,0.905}
\definecolor{mcc40}{rgb}{0.903,0.897,0.935}
\definecolor{mcc20}{rgb}{0.940,0.940,0.940}
\definecolor{mcc60}{rgb}{0.978,0.909,0.825}
\definecolor{mcc10}{rgb}{0.986,0.851,0.719}
\definecolor{mcc00}{rgb}{0.963,0.764,0.622}
\definecolor{mcc61}{rgb}{0.760,0.709,0.848}
\definecolor{mcc51}{rgb}{0.843,0.820,0.905}
\definecolor{mcc31}{rgb}{0.903,0.897,0.935}
\definecolor{mcc41}{rgb}{0.940,0.940,0.940}
\definecolor{mcc21}{rgb}{0.978,0.909,0.825}
\definecolor{mcc01}{rgb}{0.986,0.851,0.719}
\definecolor{mcc11}{rgb}{0.963,0.764,0.622}
\definecolor{mcc42}{rgb}{0.760,0.709,0.848}
\definecolor{mcc22}{rgb}{0.760,0.709,0.848}
\definecolor{mcc32}{rgb}{0.760,0.709,0.848}
\definecolor{mcc52}{rgb}{0.760,0.709,0.848}
\definecolor{mcc62}{rgb}{0.903,0.897,0.935}
\definecolor{mcc12}{rgb}{0.978,0.909,0.825}
\definecolor{mcc02}{rgb}{0.963,0.764,0.622}
\definecolor{mcc23}{rgb}{0.760,0.709,0.848}
\definecolor{mcc43}{rgb}{0.760,0.709,0.848}
\definecolor{mcc33}{rgb}{0.885,0.875,0.933}
\definecolor{mcc53}{rgb}{0.885,0.875,0.933}
\definecolor{mcc63}{rgb}{0.940,0.940,0.940}
\definecolor{mcc13}{rgb}{0.997,0.894,0.767}
\definecolor{mcc03}{rgb}{0.963,0.764,0.622}
\definecolor{mcc14}{rgb}{0.760,0.709,0.848}
\definecolor{mcc04}{rgb}{0.860,0.842,0.916}
\definecolor{mcc24}{rgb}{0.918,0.914,0.937}
\definecolor{mcc34}{rgb}{0.963,0.922,0.871}
\definecolor{mcc64}{rgb}{0.990,0.868,0.738}
\definecolor{mcc54}{rgb}{0.990,0.868,0.738}
\definecolor{mcc44}{rgb}{0.963,0.764,0.622}
\definecolor{mcc05}{rgb}{0.760,0.709,0.848}
\definecolor{mcc15}{rgb}{0.860,0.842,0.916}
\definecolor{mcc35}{rgb}{0.918,0.914,0.937}
\definecolor{mcc65}{rgb}{0.918,0.914,0.937}
\definecolor{mcc55}{rgb}{0.963,0.922,0.871}
\definecolor{mcc45}{rgb}{0.990,0.868,0.738}
\definecolor{mcc25}{rgb}{0.963,0.764,0.622}
\definecolor{mcc16}{rgb}{0.760,0.709,0.848}
\definecolor{mcc36}{rgb}{0.843,0.820,0.905}
\definecolor{mcc66}{rgb}{0.903,0.897,0.935}
\definecolor{mcc56}{rgb}{0.940,0.940,0.940}
\definecolor{mcc06}{rgb}{0.978,0.909,0.825}
\definecolor{mcc46}{rgb}{0.986,0.851,0.719}
\definecolor{mcc26}{rgb}{0.963,0.764,0.622}
\definecolor{mcc07}{rgb}{0.760,0.709,0.848}
\definecolor{mcc17}{rgb}{0.860,0.842,0.916}
\definecolor{mcc67}{rgb}{0.918,0.914,0.937}
\definecolor{mcc37}{rgb}{0.918,0.914,0.937}
\definecolor{mcc57}{rgb}{0.963,0.922,0.871}
\definecolor{mcc47}{rgb}{0.990,0.868,0.738}
\definecolor{mcc27}{rgb}{0.963,0.764,0.622}

\footnotesize
\begin{tblr}{l cccc cc cc}
    \toprule
                         & \SetCell[c=4]{c}{Error $\downarrow$} &   &   &   & \SetCell[c=2]{c}{Compression $\downarrow$} &   & \SetCell[c=2]{c}{Decompression $\downarrow$} &   \\
                           \cmidrule[lr]{2-5}                                   \cmidrule[lr]{6-7}                                    \cmidrule[lr]{8-9}
                         & \SetCell[c=2]{c}{Maximum} &   & \SetCell[c=2]{c}{Average} &   &        &       &        &                    \\
                           \cmidrule[lr]{2-3}                     \cmidrule[lr]{4-5}
    Method               & Domain & Range & Domain & Range & Domain & Range & Unpack & $\mathrm{norm}_2$ \\
    \midrule
    $\lTwoI$ & \SetCell{bg=mcc00} $0.154$ \cmark & \SetCell{bg=mcc01} $0.0963$ \cmark & \SetCell{bg=mcc02} $0.0532$ & \SetCell{bg=mcc03} $0.0523$ & \SetCell{bg=mcc04} $5.47$ & \SetCell{bg=mcc05} $47.7$ & \SetCell{bg=mcc06} $4.01$ & \SetCell{bg=mcc07} $4.01$ \\
    $\lInf$ & \SetCell{bg=mcc10} $0.121$ \cmark & \SetCell{bg=mcc11} $0.120$ \cmark & \SetCell{bg=mcc12} $0.0494$ & \SetCell{bg=mcc13} $0.0488$ & \SetCell{bg=mcc14} $3.98$ & \SetCell{bg=mcc15} $52.5$ & \SetCell{bg=mcc16} $3.23$ & \SetCell{bg=mcc17} $5.08$ \\
    $\lInfT$ ($\tan$) & \SetCell{bg=mcc20} $0.0942$ \cmark & \SetCell{bg=mcc21} $0.0939$ \cmark & \SetCell{bg=mcc22} $0.0470$ & \SetCell{bg=mcc23} $0.0462$ & \SetCell{bg=mcc24} $13.5$ & \SetCell{bg=mcc25} $119$ & \SetCell{bg=mcc26} $8.74$ & \SetCell{bg=mcc27} $12.1$ \\
    $\lInfT$ (Remez3) & \SetCell{bg=mcc30} $0.0935$ \cmark & \SetCell{bg=mcc31} $0.0924$ \cmark & \SetCell{bg=mcc32} $0.0470$ & \SetCell{bg=mcc33} $0.0463$ & \SetCell{bg=mcc34} $23.7$ & \SetCell{bg=mcc35} $90.4$ & \SetCell{bg=mcc36} $3.94$ & \SetCell{bg=mcc37} $6.14$ \\
    $\lInfT$ (Remez5) & \SetCell{bg=mcc40} $0.0941$ \cmark & \SetCell{bg=mcc41} $0.0932$ \cmark & \SetCell{bg=mcc42} $0.0470$ & \SetCell{bg=mcc43} $0.0462$ & \SetCell{bg=mcc44} $42.0$ & \SetCell{bg=mcc45} $114$ & \SetCell{bg=mcc46} $4.28$ & \SetCell{bg=mcc47} $7.27$ \\
    $\lInfT$ (Remez3-Opt-Domain) & \SetCell{bg=mcc50} $0.0926$ \cmark & \SetCell{bg=mcc51} $0.0912$ \cmark & \SetCell{bg=mcc52} $0.0470$ & \SetCell{bg=mcc53} $0.0463$ & \SetCell{bg=mcc54} $23.8$ & \SetCell{bg=mcc55} $90.7$ & \SetCell{bg=mcc56} $3.97$ & \SetCell{bg=mcc57} $6.15$ \\
    $\lInfT$ (Remez3-Opt-Range) & \SetCell{bg=mcc60} $0.107$ \xmark & \SetCell{bg=mcc61} $0.0818$ \cmark & \SetCell{bg=mcc62} $0.0483$ & \SetCell{bg=mcc63} $0.0474$ & \SetCell{bg=mcc64} $23.8$ & \SetCell{bg=mcc65} $90.4$ & \SetCell{bg=mcc66} $3.95$ & \SetCell{bg=mcc67} $6.14$ \\
    \bottomrule
\end{tblr}


==> tabs/Measurements4D_Merged.tex <==
% Merged from Measurements4D.tex and Measurements4D_Opt.tex -- colors recomputed jointly across all rows. Edits here will be overwritten if regenerated.
\definecolor{mcc50}{rgb}{0.550,0.606,0.686}
\definecolor{mcc30}{rgb}{0.607,0.649,0.721}
\definecolor{mcc40}{rgb}{0.667,0.692,0.742}
\definecolor{mcc20}{rgb}{0.730,0.735,0.748}
\definecolor{mcc60}{rgb}{0.785,0.780,0.757}
\definecolor{mcc10}{rgb}{0.875,0.855,0.732}
\definecolor{mcc00}{rgb}{1.000,0.961,0.672}
\definecolor{mcc61}{rgb}{0.550,0.606,0.686}
\definecolor{mcc51}{rgb}{0.607,0.649,0.721}
\definecolor{mcc31}{rgb}{0.667,0.692,0.742}
\definecolor{mcc41}{rgb}{0.730,0.735,0.748}
\definecolor{mcc21}{rgb}{0.785,0.780,0.757}
\definecolor{mcc01}{rgb}{0.875,0.855,0.732}
\definecolor{mcc11}{rgb}{1.000,0.961,0.672}
\definecolor{mcc22}{rgb}{0.550,0.606,0.686}
\definecolor{mcc32}{rgb}{0.550,0.606,0.686}
\definecolor{mcc42}{rgb}{0.550,0.606,0.686}
\definecolor{mcc52}{rgb}{0.550,0.606,0.686}
\definecolor{mcc62}{rgb}{0.667,0.692,0.742}
\definecolor{mcc12}{rgb}{0.785,0.780,0.757}
\definecolor{mcc02}{rgb}{1.000,0.961,0.672}
\definecolor{mcc23}{rgb}{0.550,0.606,0.686}
\definecolor{mcc43}{rgb}{0.550,0.606,0.686}
\definecolor{mcc33}{rgb}{0.636,0.670,0.739}
\definecolor{mcc53}{rgb}{0.636,0.670,0.739}
\definecolor{mcc63}{rgb}{0.730,0.735,0.748}
\definecolor{mcc13}{rgb}{0.813,0.802,0.762}
\definecolor{mcc03}{rgb}{1.000,0.961,0.672}
\definecolor{mcc14}{rgb}{0.550,0.606,0.686}
\definecolor{mcc04}{rgb}{0.607,0.649,0.721}
\definecolor{mcc24}{rgb}{0.667,0.692,0.742}
\definecolor{mcc34}{rgb}{0.730,0.735,0.748}
\definecolor{mcc54}{rgb}{0.785,0.780,0.757}
\definecolor{mcc64}{rgb}{0.875,0.855,0.732}
\definecolor{mcc44}{rgb}{1.000,0.961,0.672}
\definecolor{mcc05}{rgb}{0.550,0.606,0.686}
\definecolor{mcc15}{rgb}{0.619,0.657,0.728}
\definecolor{mcc35}{rgb}{0.692,0.709,0.744}
\definecolor{mcc45}{rgb}{0.763,0.762,0.754}
\definecolor{mcc25}{rgb}{0.850,0.834,0.744}
\definecolor{mcc55}{rgb}{0.850,0.834,0.744}
\definecolor{mcc65}{rgb}{1.000,0.961,0.672}
\definecolor{mcc16}{rgb}{0.550,0.606,0.686}
\definecolor{mcc06}{rgb}{0.619,0.657,0.728}
\definecolor{mcc36}{rgb}{0.619,0.657,0.728}
\definecolor{mcc46}{rgb}{0.692,0.709,0.744}
\definecolor{mcc66}{rgb}{0.763,0.762,0.754}
\definecolor{mcc56}{rgb}{0.850,0.834,0.744}
\definecolor{mcc26}{rgb}{1.000,0.961,0.672}
\definecolor{mcc07}{rgb}{0.550,0.606,0.686}
\definecolor{mcc17}{rgb}{0.607,0.649,0.721}
\definecolor{mcc37}{rgb}{0.667,0.692,0.742}
\definecolor{mcc47}{rgb}{0.730,0.735,0.748}
\definecolor{mcc67}{rgb}{0.785,0.780,0.757}
\definecolor{mcc57}{rgb}{0.875,0.855,0.732}
\definecolor{mcc27}{rgb}{1.000,0.961,0.672}

\footnotesize
\begin{tblr}{l cccc cc cc}
    \toprule
                         & \SetCell[c=4]{c}{Error $\downarrow$} &   &   &   & \SetCell[c=2]{c}{Compression $\downarrow$} &   & \SetCell[c=2]{c}{Decompression $\downarrow$} &   \\
                           \cmidrule[lr]{2-5}                                   \cmidrule[lr]{6-7}                                    \cmidrule[lr]{8-9}
                         & \SetCell[c=2]{c}{Maximum} &   & \SetCell[c=2]{c}{Average} &   &        &       &        &                    \\
                           \cmidrule[lr]{2-3}                     \cmidrule[lr]{4-5}
    Method               & Domain & Range & Domain & Range & Domain & Range & Unpack & $\mathrm{norm}_2$ \\
    \midrule
    $\lTwoI$ & \SetCell{bg=mcc00} $0.154$ \cmark & \SetCell{bg=mcc01} $0.0963$ \cmark & \SetCell{bg=mcc02} $0.0532$ & \SetCell{bg=mcc03} $0.0523$ & \SetCell{bg=mcc04} $5.47$ & \SetCell{bg=mcc05} $47.6$ & \SetCell{bg=mcc06} $3.97$ & \SetCell{bg=mcc07} $3.97$ \\
    $\lInf$ & \SetCell{bg=mcc10} $0.121$ \cmark & \SetCell{bg=mcc11} $0.120$ \cmark & \SetCell{bg=mcc12} $0.0494$ & \SetCell{bg=mcc13} $0.0488$ & \SetCell{bg=mcc14} $4.00$ & \SetCell{bg=mcc15} $52.6$ & \SetCell{bg=mcc16} $3.23$ & \SetCell{bg=mcc17} $5.09$ \\
    $\lInfTan$ & \SetCell{bg=mcc20} $0.0942$ \cmark & \SetCell{bg=mcc21} $0.0939$ \cmark & \SetCell{bg=mcc22} $0.0470$ & \SetCell{bg=mcc23} $0.0462$ & \SetCell{bg=mcc24} $13.5$ & \SetCell{bg=mcc25} $119$ & \SetCell{bg=mcc26} $8.67$ & \SetCell{bg=mcc27} $12.0$ \\
    $\lInfT$ (Remez3) & \SetCell{bg=mcc30} $0.0935$ \cmark & \SetCell{bg=mcc31} $0.0924$ \cmark & \SetCell{bg=mcc32} $0.0470$ & \SetCell{bg=mcc33} $0.0463$ & \SetCell{bg=mcc34} $23.9$ & \SetCell{bg=mcc35} $91.1$ & \SetCell{bg=mcc36} $3.97$ & \SetCell{bg=mcc37} $6.15$ \\
    $\lInfT$ (Remez5) & \SetCell{bg=mcc40} $0.0941$ \cmark & \SetCell{bg=mcc41} $0.0932$ \cmark & \SetCell{bg=mcc42} $0.0470$ & \SetCell{bg=mcc43} $0.0462$ & \SetCell{bg=mcc44} $42.0$ & \SetCell{bg=mcc45} $114$ & \SetCell{bg=mcc46} $4.36$ & \SetCell{bg=mcc47} $7.62$ \\
    $\lInfT$ (Remez3-Opt-Domain) & \SetCell{bg=mcc50} $0.0926$ \cmark & \SetCell{bg=mcc51} $0.0912$ \cmark & \SetCell{bg=mcc52} $0.0470$ & \SetCell{bg=mcc53} $0.0463$ & \SetCell{bg=mcc54} $27.2$ & \SetCell{bg=mcc55} $119$ & \SetCell{bg=mcc56} $6.73$ & \SetCell{bg=mcc57} $9.73$ \\
    $\lInfT$ (Remez3-Opt-Range) & \SetCell{bg=mcc60} $0.107$ \xmark & \SetCell{bg=mcc61} $0.0818$ \cmark & \SetCell{bg=mcc62} $0.0483$ & \SetCell{bg=mcc63} $0.0474$ & \SetCell{bg=mcc64} $32.5$ & \SetCell{bg=mcc65} $120$ & \SetCell{bg=mcc66} $6.27$ & \SetCell{bg=mcc67} $9.27$ \\
    \bottomrule
\end{tblr}


==> tabs/TableGenerator.tex <==

\begin{tabular}{@{}lllll@{}}
\toprule
Head        & Head           & Head & Head & Head \\ \midrule
1           & 2              & 3    & 4    & 5    \\
A           & B              & C    & D    & E    \\
\textless{} & \textgreater{} & !    & X    & \#   \\ \bottomrule
\end{tabular}


==> tabs/gaussian_splats_quality.tex <==
% Tabular only; the float and its caption are in secs/B5results.tex.
% Numbers from QuaternionCompression/doc/paper_gaussian_splatting/GaussianRotationSection.ipynb.
\begin{tabular}{@{}llrrrr@{}}
\toprule
 &  & \multicolumn{2}{c}{Quaternion ($^\circ$)} & \multicolumn{2}{c}{Image} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
\begin{tabular}[b]{@{}l@{}}Budget\\(bits)\end{tabular} & Method & Max $\downarrow$ & Mean $\downarrow$ & PSNR (dB) $\uparrow$ & FLIP $\downarrow$ \\
\midrule
\multirow{4}{*}{30} & Exp & 0.3034 & 0.1533 & 45.90 & 0.02871 \\
 & Exp-Ours & 0.1519 & 0.0771 & 45.99 & 0.02856 \\
 & $\lTwoI$ & 0.1197 & 0.0647 & \textbf{\boldmath 46.01} & 0.02852 \\
 & $\lInfCub$ & \textbf{\boldmath 0.1059} & \textbf{\boldmath 0.0584} & \textbf{\boldmath 46.01} & \textbf{\boldmath 0.02851} \\
\midrule
\multirow{4}{*}{24} & Exp & 1.2016 & 0.6117 & 44.62 & 0.03141 \\
 & Exp-Ours & 0.6028 & 0.3053 & 45.61 & 0.02932 \\
 & $\lTwoI$ & 0.4943 & 0.2593 & 45.76 & 0.02909 \\
 & $\lInfCub$ & \textbf{\boldmath 0.4086} & \textbf{\boldmath 0.2334} & \textbf{\boldmath 45.83} & \textbf{\boldmath 0.02897} \\
\midrule
\multirow{4}{*}{16} & Exp & 7.7409 & 3.9188 & 35.01 & 0.06527 \\
 & Exp-Ours & 3.8784 & 1.9577 & 39.45 & 0.04399 \\
 & $\lTwoI$ & 2.9812 & 1.6464 & 40.91 & 0.04013 \\
 & $\lInfCub$ & \textbf{\boldmath 2.6355} & \textbf{\boldmath 1.4818} & \textbf{\boldmath 41.68} & \textbf{\boldmath 0.03822} \\
\bottomrule
\end{tabular}


==> tabs/gaussian_splats_time.tex <==
% Generated by the Gaussian rotation notebook; do not edit.
\begin{table}[t]
\centering
\small
\caption{Decompression cost on the GPU, averaged over the \num{3} scenes. Device: \nvidiaGpu{}.}
\label{tab:gs-rotation-decode}
\begin{tabular}{@{}llrr@{}}
\toprule
Budget & Method & Decode (\unit{\milli\second}) & Render (\unit{\milli\second}) \\
\midrule
\multirow{4}{*}{30 (128 total)} & Exp & 0.496 & 11.834 \\
 & Exp-Ours & 0.501 & \textbf{\boldmath 11.818} \\
 & $\ell_{2\mathrm{I}}$ & \textbf{\boldmath 0.495} & 11.851 \\
 & $\lInfCub$ & 0.516 & 11.845 \\
\midrule
\multirow{4}{*}{24 (128 total)} & Exp & \textbf{\boldmath 0.489} & 11.853 \\
 & Exp-Ours & 0.495 & \textbf{\boldmath 11.825} \\
 & $\ell_{2\mathrm{I}}$ & 0.499 & 11.872 \\
 & $\lInfCub$ & 0.499 & 11.858 \\
\midrule
\multirow{4}{*}{16 (128 total)} & Exp & 0.484 & 11.878 \\
 & Exp-Ours & \textbf{\boldmath 0.474} & \textbf{\boldmath 11.839} \\
 & $\ell_{2\mathrm{I}}$ & 0.481 & 11.883 \\
 & $\lInfCub$ & 0.487 & 11.876 \\
\midrule
\multirow{2}{*}{10 (96 total)} & Exp & \textbf{\boldmath 0.499} & \textbf{\boldmath 10.609} \\
 & $\lInfCub$ & 0.521 & 10.633 \\
\bottomrule
\end{tabular}
\end{table}

==> tabs/mixamo_quality.tex <==
% Tabular only; the float and its caption are in secs/B5results.tex.
% Numbers from ozz-animation-liw/paper/mixamo_compression/mixamo_compression.ipynb.
\begin{tabular}{@{}lrcrrr@{}}
\toprule
 &  &  &  & \multicolumn{2}{c}{Geodesic error ($^\circ$)} \\
\cmidrule(lr){5-6}
Method & Bits & \begin{tabular}[b]{@{}c@{}}Sign \\ bit\end{tabular} & States & Max $\downarrow$ & Mean $\downarrow$ \\
\midrule
Ozz & 48 & yes & \num{32768} & 0.00909 & 0.00187 \\
$\lInfCub$-48 & 48 & yes & \num{32768} & 0.00203 & 0.00129 \\
$\lInfCub$-40 & 40 & yes & \num{5160} & 0.01296 & 0.00823 \\
\midrule
$\lInfCub$-48 & 48 & no & \num{41285} & \textbf{\boldmath 0.00161} & \textbf{\boldmath 0.00065} \\
$\lInfCub$-40 & 40 & no & \num{6501} & 0.01020 & 0.00405 \\
\bottomrule
\end{tabular}


==> tabs/reduced_gaussian_geometry_test.tex <==
%% Generated by the Gaussian rotation notebook; do not edit.
%\begin{table}[t]
%\centering
%\small
%\caption{Image quality with reduced Gaussian geometry (16-bit rotation encoding) on \num{3} scene(s), averaged over test views. Higher PSNR and lower FLIP are better.}
%\label{tab:reduced-gaussian-geometry-test}
%\begin{tabular}{@{}llrr@{}}
%\toprule
 %&  & \multicolumn{2}{c}{Image} \\
%\cmidrule(lr){3-4}
%SPP & Method & PSNR (dB) & FLIP \\
%\midrule
%\multirow{2}{*}{1} & Exp & 19.23 & 0.15300 \\
 %& $\lInfCub$ & \textbf{\boldmath 19.30} & \textbf{\boldmath 0.14939} \\
%\midrule
%\multirow{2}{*}{4} & Exp & 24.47 & 0.12458 \\
 %& $\lInfCub$ & \textbf{\boldmath 24.68} & \textbf{\boldmath 0.12053} \\
%\midrule
%\multirow{2}{*}{16} & Exp & 28.42 & 0.11501 \\
 %& $\lInfCub$ & \textbf{\boldmath 28.94} & \textbf{\boldmath 0.11094} \\
%\midrule
%\multirow{2}{*}{64} & Exp & 30.46 & 0.11235 \\
 %& $\lInfCub$ & \textbf{\boldmath 31.29} & \textbf{\boldmath 0.10830} \\
%\midrule
%\multirow{2}{*}{256} & Exp & 31.18 & 0.11167 \\
 %& $\lInfCub$ & \textbf{\boldmath 32.15} & \textbf{\boldmath 0.10763} \\
%\midrule
%\multirow{2}{*}{1024} & Exp & 31.38 & 0.11154 \\
 %& $\lInfCub$ & \textbf{\boldmath 32.40} & \textbf{\boldmath 0.10750} \\
%\bottomrule
%\end{tabular}
%\end{table}


% Generated by the Gaussian rotation notebook; do not edit.
\begin{table}[t]
\centering
\small
\caption{Image quality with reduced Gaussian geometry (10-bit rotation) on \num{3} scene(s), averaged over test views. Higher PSNR and lower FLIP are better.}
\label{tab:reduced-gaussian-geometry-test}
\begin{tabular}{@{}llrr@{}}
\toprule
 &  & \multicolumn{2}{c}{Image} \\
\cmidrule(lr){3-4}
SPP & Method & PSNR (dB) & FLIP \\
\midrule
\multirow{2}{*}{1} & Exp & 18.67 & 0.17833 \\
 & $\lInfCub$ & \textbf{\boldmath 19.41} & \textbf{\boldmath 0.14190} \\
\midrule
\multirow{2}{*}{4} & Exp & 22.78 & 0.15309 \\
 & $\lInfCub$ & \textbf{\boldmath 24.75} & \textbf{\boldmath 0.10486} \\
\midrule
\multirow{2}{*}{16} & Exp & 25.09 & 0.14437 \\
 & $\lInfCub$ & \textbf{\boldmath 28.95} & \textbf{\boldmath 0.08865} \\
\midrule
\multirow{2}{*}{64} & Exp & 25.97 & 0.14183 \\
 & $\lInfCub$ & \textbf{\boldmath 31.32} & \textbf{\boldmath 0.08298} \\
\midrule
\multirow{2}{*}{256} & Exp & 26.22 & 0.14117 \\
 & $\lInfCub$ & \textbf{\boldmath 32.21} & \textbf{\boldmath 0.08136} \\
\midrule
\multirow{2}{*}{1024} & Exp & 26.29 & 0.14104 \\
 & $\lInfCub$ & \textbf{\boldmath 32.47} & \textbf{\boldmath 0.08098} \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/skinned_frame_time.tex <==
% Tabular only; the float and its caption are in secs/B5results.tex.
% Numbers from ozz-animation-liw/paper/skinned_benchmark/skinned_benchmark.ipynb (rendered runs, 1024 characters).
\begin{tabular}{@{}llrrr@{}}
\toprule
Regime & Method & Sampling $\downarrow$ & ns/joint $\downarrow$ & Change $\downarrow$ \\
\midrule
\multirow{3}{*}{\shortstack[l]{\qty{60}{\hertz}\\playback}}
 & $\lTwoI$-48 & \qty{5.151}{\milli\second} & 75.1 & --- \\
 & $\lInfCub$-48 & \qty{4.568}{\milli\second} & 66.6 & \qty{-11.3}{\percent} \\
 & $\lInfCub$-40 & \textbf{\qty[detect-weight]{4.500}{\milli\second}} & \textbf{\boldmath 65.6} & \textbf{\qty[detect-weight]{-12.6}{\percent}} \\
\bottomrule
\end{tabular}


==> tabs/stripify_table.tex <==
\footnotesize
\begin{tblr}[b]{lccc}
    \toprule                                        
                     & \textbf{Gurobi} & \textbf{SCIP}       & ETA\\
\midrule                                    
\textbf{computation time}     & 122.46\,s    & 8,122.56\,s & 10.52\,s   \\
{GTS render time} & 1.58\,ms     & 1.58\,ms    & 0.59\,ms \\
{GTS restarts}    & 123,784      & 123,784     & 185,480\\
\textbf{degenerate triangles} & 2,132      & 495,136     & 741,920\\
\textbf{additional meshlets}  & 1 / 12412   & 123  & 4 / 75,413\\
\bottomrule                                    
\end{tblr}


